Impact of Feature Selection on Micro-Text Classification

Social media datasets, especially Twitter tweets, are popular in the field of text classification. Tweets are a valuable source of micro-text (sometimes referred to as "micro-blogs"), and have been studied in domains such as sentiment analysis, recommendation systems, spam detection, clustering, among others. Tweets often include keywords referred to as "Hashtags" that can be used as labels for the tweet. Using tweets encompassing 50 labels, we studied the impact of word versus character-level feature selection and extraction on different learners to solve a multi-class classification task. We show that feature extraction of simple character-level groups performs better than simple word groups and pre-processing methods like normalizing using Porter's Stemming and Part-of-Speech ("POS")-Lemmatization.

==> ref.tex <==
\begin{thebibliography}{9}
\bibitem{atc} 
Sebastiani, Fabrizio. ``Machine learning in automated text categorization.'' ACM computing surveys (CSUR) 34.1 (2002): 1-47.
 
\bibitem{tclass} 
Aggarwal, Charu C., and ChengXiang Zhai. ``A survey of text classification algorithms.'' Mining Text Data. Springer US, 2012. 163-222.
 
\bibitem{dclass} 
Sriram, Bharath, et al. ``Short text classification in twitter to improve information filtering.'' Proceedings of the 33rd International ACM SIGIR Conference on Research and Development in Information Retrieval. ACM, 2010.

\bibitem{bigram}
Wang, Sida, and Christopher D. Manning. ``Baselines and bigrams: Simple, good sentiment and topic classification.'' Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics: Short Papers-Volume 2. Association for Computational Linguistics, 2012.

\bibitem{wnorm}
Toman, Michal, Roman Tesar, and Karel Jezek. ``Influence of word normalization on text classification.'' Proceedings of InSciT 4 (2006): 354-358.

\bibitem{SVMexp}
Joachims, Thorsten. ``Text categorization with support vector machines: Learning with many relevant features.'' European Conference on Machine Learning. Springer Berlin Heidelberg, 1998.

\bibitem{sklearn}
Pedregosa, Fabian, et al. ``Scikit-learn: Machine learning in Python.'' Journal of Machine Learning Research 12.  Oct (2011): 2825-2830.

\bibitem{fw1}
Kim, Yoon. ``Convolutional neural networks for sentence classification.'' arXiv preprint arXiv:1408.5882 (2014).]

\bibitem{fw2}
Tang, Duyu, et al. ``Coooolll: A deep learning system for Twitter sentiment classification.'' Proceedings of the 8th International Workshop on Semantic Evaluation (SemEval 2014). 2014.

\end{thebibliography}

